Quality-Diversity through AI Feedback

In many text-generation problems, users may prefer not only a single response, but a diverse range of high-quality outputs from which to choose. Quality-diversity (QD) search algorithms aim at such outcomes, by continually improving and diversifying a population of candidates. However, the applicability of QD to qualitative domains, like creative writing, has been limited by the difficulty of algorithmically specifying measures of quality and diversity. Interestingly, recent developments in language models (LMs) have enabled guiding search through AI feedback, wherein LMs are prompted in natural language to evaluate qualitative aspects of text. Leveraging this development, we introduce Quality-Diversity through AI Feedback (QDAIF), wherein an evolutionary algorithm applies LMs to both generate variation and evaluate the quality and diversity of candidate text. When assessed on creative writing domains, QDAIF covers more of a specified search space with high-quality samples than do non-QD controls. Further, human evaluation of QDAIF-generated creative texts validates reasonable agreement between AI and human evaluation. Our results thus highlight the potential of AI feedback to guide open-ended search for creative and original solutions, providing a recipe that seemingly generalizes to many domains and modalities. In this way, QDAIF is a step towards AI systems that can independently search, diversify, evaluate, and improve, which are among the core skills underlying human society's capacity for innovation.

==> tables/main/few_shot/human_eval_agreement.tex <==
\begin{table}[!t]
\caption{Alignment of bin assignment between humans and AI Feedback}
\label{table:few_shots_3}
\begin{center}
\begin{tabular}{cccc}
\toprule
zero-shot & 2-shot & 4-shot & 8-shot\\
80.0\% & 50.0\% & 66.7\% & 56.7\% \\
\bottomrule
\end{tabular}
\end{center}
\end{table}

==> tables/main/few_shot/human_eval_quality.tex <==
\begin{table}[!t]
\caption{Quality scores from human study.}
\label{table:few_shots_2}
\begin{center}
\begin{tabular}{cccc}
\toprule
zero-shot & 2-shot & 4-shot & 8-shot\\
3.43 & 3.10 & 3.93 & 4.03 \\
\bottomrule
\end{tabular}
\end{center}
\end{table}

==> tables/main/init_compare_human_eval.tex <==
\begin{table}[!t]
\caption{\andrew{TODO: move Zero-Shot Init to separate table for dedicated comparison, for Seeded comparisons, keep LMX-Near, for Zero-Shot Init table, maybe LMX-Replace}Mean stats, human eval scores of QDAIF with different search initialization methods. \andrew{add average of all stories. multiply human QD scores by 5}}
\label{table:mean_human_eval_init_method}
\centering
\small
\begin{tabular}{lcccc}
\toprule
\textbf{Method} &
\textbf{QD score} & \textbf{Quality} & \textbf{H-AI agreement} & \textbf{H agreement }  \\
\midrule
Zero-Shot Init & 0.383 & 2.233 & 0.600 & 0.600  \\
Seeded Init & 0.772 & 3.900 & 0.833 & 0.800  \\
\bottomrule
\end{tabular}
\end{table}



==> tables/main/old_aif_vs_baseline_human_eval.tex <==
\begin{table}[!t]
\caption{\andrew{TODO: move to appendix, and make more compact.} Stats for different creative writing domains, human eval scores, Baselines vs QDAIF. The QD score presented here is based on subjective evaluation results, not computed. \andrew{add average of all stories. multiply human QD scores by 5}}
\label{table:human_eval_baselines_vs_aif}
\centering
\small
\begin{tabular}{lcccccc}
\toprule
\textbf{Method} &
\textbf{QD score} & \textbf{QD range} & \textbf{Quality} & \textbf{Q Range} & \textbf{H-AI agreement} & \textbf{H agreement }  \\
\midrule
\multicolumn{7}{c}{Opinions} \\
\midrule
Baseline 1 & 1.000 & 0.000 & 5.000 & 0.000 & 0.700 & 0.800  \\ 
Baseline 2 & 0.728 & 0.056 & 3.600 & 0.800 & 0.700 & 0.800  \\ 
Baseline 3 & 0.600 & 0.267 & 3.600 & 0.800 & 0.700 & 0.800  \\ 
Baseline 4 & 0.750 & 0.300 & 3.800 & 1.200 & 0.600 & 1.000  \\ 
AIF, Near, Generated & 0.350 & 0.300 & 1.700 & 1.400 & 0.800 & 1.000  \\ 
AIF, Near, Seed & 0.617 & 0.167 & 3.200 & 1.200 & 1.000 & 1.000  \\ 
AIF, Replace, Generated & 0.833 & 0.267 & 4.300 & 1.000 & 0.600 & 0.600  \\ 
AIF, Replace, Seed & 0.739 & 0.078 & 3.700 & 0.600 & 0.700 & 0.800 \\ 
\midrule
\multicolumn{7}{c}{Stories (Genre)} \\
\midrule
Baseline 1 & 0.650 & 0.167 & 3.400 & 1.600 & 1.000 & 1.000  \\ 
Baseline 2 & 0.861 & 0.056 & 4.300 & 0.600 & 0.700 & 0.800  \\ 
Baseline 3 & 0.683 & 0.100 & 3.400 & 0.800 & 0.700 & 0.400  \\ 
Baseline 4 & 0.600 & 0.267 & 2.900 & 1.400 & 0.700 & 0.800  \\ 
AIF, Near, Generated & 0.200 & 0.000 & 1.400 & 0.400 & 0.400 & 0.600  \\ 
AIF, Near, Seed & 0.767 & 0.133 & 3.700 & 0.600 & 0.800 & 1.000  \\ 
AIF, Replace, Generated & 0.286 & 0.006 & 1.500 & 0.200 & 0.500 & 0.800  \\ 
AIF, Replace, Seed & 0.683 & 0.100 & 3.500 & 0.600 & 0.900 & 0.800 \\ 
\midrule
\multicolumn{7}{c}{Stories (Ending)} \\
\midrule
Baseline 1 & 0.650 & 0.167 & 4.000 & 0.400 & 0.700 & 0.800  \\ 
Baseline 2 & 0.500 & 0.200 & 2.600 & 0.800 & 0.700 & 0.400  \\ 
Baseline 3 & 0.533 & 0.000 & 2.900 & 1.400 & 0.800 & 0.600  \\ 
Baseline 4 & 0.600 & 0.400 & 3.900 & 0.600 & 0.600 & 0.400  \\ 
AIF, Near, Generated & 0.600 & 0.200 & 3.600 & 0.800 & 0.600 & 0.200  \\ 
AIF, Near, Seed & 0.933 & 0.133 & 4.800 & 0.400 & 0.700 & 0.400  \\ 
AIF, Replace, Generated & 0.500 & 0.333 & 2.600 & 1.600 & 1.000 & 1.000  \\ 
AIF, Replace, Seed & 0.867 & 0.267 & 4.200 & 1.600 & 0.800 & 0.800 \\ 
\bottomrule
\end{tabular}
\end{table}

==> tables/main/scaling_generation/human_eval_agreement.tex <==
\begin{table}[!t]
\caption{Alignment of bin assignment between humans and AI Feedback}
\label{table:few_shots_3}
\begin{center}
\begin{tabular}{ccc}
\toprule
13B & 30B & 70B\\
80.0\% & 73.3\% & 73.3\% \\
\bottomrule
\end{tabular}
\end{center}
\end{table}

==> tables/main/scaling_generation/human_eval_quality.tex <==
\begin{table}[!t]
\caption{Quality scores from human study.}
\label{table:few_shots_2}
\begin{center}
\begin{tabular}{ccc}
\toprule
13B & 30B & 70B\\
3.43 & 3.60 & 4.03 \\
\bottomrule
\end{tabular}
\end{center}
\end{table}
